Efficient-NeRF2NeRF: Streamlining Text-Driven 3D Editing with Multiview Correspondence-Enhanced Diffusion Models

The advancement of text-driven 3D content editing has been blessed by the progress from 2D generative diffusion models. However, a major obstacle hindering the widespread adoption of 3D content editing is its time-intensive processing. This challenge arises from the iterative and refining steps required to achieve consistent 3D outputs from 2D image-based generative models. Recent state-of-the-art methods typically require optimization time ranging from tens of minutes to several hours to edit a 3D scene using a single GPU. In this work, we propose that by incorporating correspondence regularization into diffusion models, the process of 3D editing can be significantly accelerated. This approach is inspired by the notion that the estimated samples during diffusion should be multiview-consistent during the diffusion generation process. By leveraging this multiview consistency, we can edit 3D content at a much faster speed. In most scenarios, our proposed technique brings a 10$\times$ speed-up compared to the baseline method and completes the editing of a 3D scene in 2 minutes with comparable quality.

==> abs.tex <==
\begin{abstract}
Recent advancements in text-driven 2D image editing have significantly enhanced the performance of 3D editing. The majority of existing methods for 3D editing suffer from slow processing times due to the need for iteration and refinement in order to produce 3D consistent results from 2D image editing models. In this paper, we propose a novel approach to address this issue by incorporating correspondence regularization into diffusion models, thereby ensuring multiview consistency in the edited images. This regularization is inspired by the insight that the estimated noise should exhibit multiview consistency throughout the denoising process in diffusion. By leveraging the multiview consistent editing results, we can directly update the 3D content with our generated images, thereby achieving highly efficient editing performance. Our proposed method is capable of completing the editing process in under 2 minutes in the majority of cases, a significant improvement in efficiency compared to existing methods.
\end{abstract}

==> model.tex <==
\section{Preliminaries}
\llcao{Shall we rename this section as "Problem Definition", and only talk about (a) NeRF (b) Input and output of your problem?

coz I am afraid people may either get confused by the many equations, or skip this section if they think they understand these background.}
\paragraph{Diffusion Models.} 
Diffusion models \cite{song2019generative,ddpm,ddim,croitoru2023diffusion} aim to approximate a given data distribution $q(\bm{x}_0)$ by learning a model distribution $p_{\theta}(\bm{x}_0)$ that is both a good approximation of $q(\bm{x}_0)$ and allows for efficient sampling. A significant contribution in this field is the development of Denoising Diffusion Probabilistic Models (DDPMs \cite{sohl2015deep,ddpm,song2020score}), which are a type of latent variable models described by the following form:
\begin{equation}
    p_\theta(\bm{x}_0) = \int p_\theta(\bm{x}_{0:T}) \mathrm{d} \bm{x}_{1:T} \label{eq:gen0}
\end{equation}
where $\bm{x}_1, \ldots, \bm{x}_T$ are latent variables in the same sample space as $\bm{x}_0$ (denoted as $\mathcal{X}$), and $p_\theta(\bm{x}_{0:T}) := p_\theta(\bm{x}_T) \prod_{t=1}^{T} p^{(t)}_\theta(\bm{x}_{t-1} | \bm{x}_t)$. 
In DDPM \cite{ddpm}, we have $p(\bm{x}_T)=\mathcal{N}(\bm{x}_T; \mathbf{0}, \mathbf{I})$ and $p_\theta(\bm{x}_{t-1}|\bm{x}_t)=\mathcal{N}(\bm{x}_{t-1};\mu_\theta(\bm{x}_t,t),\sigma^2_t \mathbf{I})$, where the trainable component $\mu_\theta(\bm{x}_t,t)$ has the time-dependent constant variance $\sigma^2_t$.
Forward process is then defined to learn $\mu_\theta$ as
$q(\bm{x}_{1:T}|\bm{x}_0)=\prod_{t=1}^{T} q(\bm{x}_t|\bm{x}_{t-1}),$
where $q(\bm{x}_t|\bm{x}_{t-1})=\mathcal{N}(\bm{x}_t;\sqrt{1-\beta_t} \bm{x}_{t-1},\beta_t \mathbf{I})$ with $\beta_t$ as predefined constants. Next, in DDPM we have
\begin{equation}
    \mu_\theta(\bm{x}_t,t)=\frac{1}{\sqrt{\alpha}_t}\left(\bm{x}_t - \frac{\beta_t}{\sqrt{1-\bar{\alpha}_t}} \bm{\epsilon}_\theta (\bm{x}_t, t)\right),
    \label{eq:diffusion}
\end{equation}
where $\alpha_t$ and $\bar{\alpha}_t$ are constants derived from $\beta_t$ and $\bm{\epsilon}_\theta$ is a noise predictor, usually parameterized by neural networks.
In image generation tasks, the generation can be conditioned on inputs like text or reference images, and we have 
\begin{equation}
    \bm{\epsilon}^{t}=\bm{\epsilon}_\theta(\bm{x}_t,t,\bm{c}),
    \label{eq:denoise}
\end{equation}
where $\bm{c}$ is the conditioning inputs. 

\paragraph{Radiance Fields.}
3D contents in radiance fields are represented by functions that take in spatial location $(x,y,z)$ and viewing direction $(\theta,\phi)$ and output the radiance and occupancy of that location. The radiance value and occupancy for all points along a camera ray are considered to render an image from the radiance fields. 
Volume rendering \cite{mildenhall2020nerf} facilitates the generation of radiance fields by accessing and analyzing all points present on the camera rays. Recent advancements, such as the utilization of 3D Gaussian points \cite{kerbl20233d} to parameterize a radiance field, have led to more efficient rendering pipelines. we opt to generalize the rendering process by symbolically representing it as 
\begin{equation}
    \bm{I}=\pi(\mathcal{F}, \mathbf{P}), \label{eq:render}
\end{equation}
where $\bm{I}$ is the rendered image, $\mathcal{F}$ is the radiance field, and $\mathbf{P}$ is the camera projection matrix (\ie, intrinsics and extrinsics).


\section{Our Method}
The overall framework of our proposed method is straightforward. First, we edit multiview images by the provided textual prompt. Subsequently, we proceed to update the radiance field with these edited images.

\subsection{Multiview Correspondence Regularization}
The goal of correspondence regularization is to maintain the correspondence between the multiple views of an image after editing. Our method for pursuing this objective is quite clear: \textit{we aim to ensure that the estimated noise is aligned with the inputs from the multiple views during the denoising process}. 

\begin{figure}
\scriptsize
    \centering
    \includegraphics[width=0.3\columnwidth]{fig/blind-compare/frame_00036.jpg}
    \includegraphics[width=0.3\columnwidth]{fig/blind-compare/frame_00042.jpg}
    \includegraphics[width=0.3\columnwidth]{fig/blind-compare/frame_00002.jpg}\\
    (a) Input views\\
    \includegraphics[width=0.3\columnwidth]{fig/blind-compare/blind19-0.jpg}
    \includegraphics[width=0.3\columnwidth]{fig/blind-compare/blind19-1.jpg}
    \includegraphics[width=0.3\columnwidth]{fig/blind-compare/blind19-2.jpg}\\
    (b) Enforcing multiview correspondence on all noise predictions (\cf \cref{eq:averageall})\\
    \includegraphics[width=0.3\columnwidth]{fig/blind-compare/19-0.jpg}
    \includegraphics[width=0.3\columnwidth]{fig/blind-compare/19-1.jpg}
    \includegraphics[width=0.3\columnwidth]{fig/blind-compare/19-2.jpg}\\
    (a) With our soft correspondence regularization\\
    \caption{\textbf{Multiview image editing results} of (a) input views with (b) enforcing multiview correspondence on all noise predictions, and (c) our soft correspondence regularization. (Prompt: \textit{``Turn him into Albert Einstein''}.)}
    \label{fig:blind}
\end{figure}

Without loss of generality, let us consider two views, denoted as $\bm{I}_a$ and $\bm{I}_b$, and suppose there are $K$ corresponding points denoted as $\{(_a^k, \bm{p}_b^k)\}_{k=1}^K$.
According to the definition of denoising in equation \ref{eq:denoise}, now the conditioning for editing the two images becomes $\bm{c}_a=\{\bm{c}_\text{prompt}, \bm{I}_a\}$ and $\bm{c}_b=\{\bm{c}_\text{prompt}, \bm{I}_b\}$.
For time $t$, we further have the estimated noise $\bm{\epsilon}^{t}_a$ and $\bm{\epsilon}^{t}_b$ based on the conditioning. 
Our regularization is based on a distance on the estimated noise based on the corresponding points in the input, namely correspondence distance, as defined by
\begin{equation}
    d\left(\bm{\epsilon}_a, \bm{\epsilon}_a;\{(\bm{p}_a^k, \bm{p}_b^k)\}_{k=1}^K\right) = \frac{1}{K} \sum_{k=1}^K\left(\bm{\epsilon}_a[\bm{p}_a^k]-\bm{\epsilon}_b[\bm{p}_b^k]\right),
    \label{eq:distance}
\end{equation}
where $\bm{\epsilon}^{t}[\bm{p}^k]$ means the value of $\bm{\epsilon}^{t}$ on the coordinate $\bm{p}^k$.
Our regularization can be then formulated as a loss for minimizing the distance, \ie,
\begin{equation}
    L_\text{reg}(\bm{\epsilon}_a, \bm{\epsilon}_b) = \min_{\bm{\epsilon}_a, \bm{\epsilon}_b} d\left(\bm{\epsilon}_a, \bm{\epsilon}_a;\{(\bm{p}_a^k, \bm{p}_b^k)\}_{k=1}^K\right). 
    \label{eq:reg}
\end{equation}
Incorporating the regularization loss in the retraining of the diffusion network can indeed be a viable approach. However, it is worth noting that this method may result in significant training time requirements, making it less desirable. Fortunately, there exists a closed-form solution for the regularization loss, that is,
\begin{equation}
    \overline{\bm{\epsilon}_a^t}[\bm{p}_a^k]=\overline{\bm{\epsilon}_b^t}[\bm{p}_b^k]=\frac{1}{2}\left(\bm{\epsilon}^t_a[\bm{p}_a^k]+\bm{\epsilon}^t_b[\bm{p}_b^k]\right), \forall t\in[0,T]
    \label{eq:averageall}
\end{equation}
where $\overline{\bm{\epsilon}_a^t}$ and $\overline{\bm{\epsilon}_b^t}$ are the results with the perfect multiview correspondence. \cref{eq:averageall} can be interpreted that we calculate the mean value of all correspondence pairs on the outputs from \cref{eq:denoise} and continue diffusion with \cref{eq:diffusion}.
However, directly using \cref{eq:averageall} leads to undesired over-blurred image outputs, as shown in \cref{fig:blind}(b).

The occurrence of blurred outcomes in \cref{fig:blind}(b) can be comprehended. This is predominantly due to the presence of noise in the pairs of multiview correspondences (\ie, $\{(\bm{p}_a^k, \bm{p}_b^k)\}_{k=1}^K$). This noise can arise from either imprecise estimation of correspondences or due to the diffusion backbone we have employed, which relies on downsampling in the latent space. Even if the pixel-level correspondence appears to be reliable, it does not guarantee accurate correspondence in the latent space. Furthermore, there may exist instances where strict correspondence is lacking in the latent space. In cases where the correspondence is noisy, the application of regularization will result in a blurred effect, as it produces an averaged outcome across different patches.
We propose to soften the regularization in the following section to address the undesired blurry outputs.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{fig/average-step.pdf}
    \caption{\textbf{Impact of the regularization ending step $T_\text{end}$}. Moving the regularization to early steps can avoid unwanted blurriness in the generation. (Prompt: \textit{``Give him a cowboy hat''}.)}
    \label{fig:average-step}
\end{figure*}

\subsection{Soft Regularization}
The cause of the blurred generation can be attributed to an excessively strong regularization. Thus, it is natural to consider decreasing the strength of regularization in the diffusion process. Our insight is that this reduction in regularization should preserve the majority of the semantics without the necessity of retaining all image details. For example, if we want to edit human facial images, while maintaining the multiview alignment of the facial structure is essential, inconsistencies in details such as wrinkles across different views may not be of significant concern.

Drawing on previous research \cite{meng2021sdedit}, which suggests that diffusion models primarily focus on capturing the overall structure during the initial denoising stages and pay more attention to finer details in subsequent stages, we propose to apply \cref{eq:averageall} solely to the early steps of the diffusion process. Formally, we introduce a threshold, denoted as $T_\text{end}$, which replaces $T$ in \cref{eq:averageall}. For denoising steps beyond $T_\text{end}$, no regularization is employed, and the denoising steps are carried out as per the standard procedure outlined in \cref{eq:denoise}.

In Figure 1, we present the visual representation to demonstrate the influence of various selections of $T_{\text{end}}$. The level of indistinctness grows with the increase in $T_{\text{end}}$. Empirically, we found that by setting $T_{\text{end}}$ to 10, we achieve favorable multiview-consistent editings. Consequently, we have employed this particular value for all of our experiments using the InstructPix2Pix \cite{brooks2023instructpix2pix}.

\subsection{Updating Radiance Fields}
By utilizing the multiview images obtained by regularized diffusion in the previous section, the process of updating the radiance fields becomes straightforward. First, we follow InstructNeRF2NeRF and sample a batch of $N$ training cameras $\{\mathbf{P}_n\}_{n=1}^N$. A set of images is first rendered as in \cref{eq:render}, then we apply multiview correspondence regularized 2D image editing on it. Next, with the same training cameras $\{\mathbf{P}_n\}_{n=1}^N$, we randomly render image patches with these cameras, and sample corresponding patches from the generated images in the previous step. Here, we slightly abuse the notation between images and patches, and denote the rendered patches as $\bm{I}_n$ and the corresponding edited patches as $\bm{I}_n^{\mathrm{gen}}$.
However, direct training with $\bm{I}_n^{\mathrm{gen}}$ leads to artifacts, which arise from the presence of inconsistent areas since the regularization improves consistency but is not perfect. Therefore, we propose to leverage a loss function that is not sensitive to multiview inconsistency, and through empirical analysis, we find that the style loss based on the Gram matrix \cite{gatys2016image} is an excellent candidate for this purpose. The total training loss is then
\begin{equation}
    L = \frac{1}{N}\sum_{n=1}^N\left( (\bm{I}_n-\bm{I}_n^{\mathrm{gen}})^2 + \lambda (G(\bm{I}_n)-G(\bm{I}_n^{\mathrm{gen}}))^2 \right),
    \label{eq:loss}
\end{equation}
where $G(\cdot)$ is the Gram matrix of the input, and $\lambda$ is set to 0.1 in our experiments empirically.
